Anti-Backdoor Coreset Selection via Cumulative Entropy

Recent training-time defenses against neural backdoors isolate a benign subset from poisoned training data, to learn a backdoor-free model from it. In this paper, we formulate this defense strategy as a coreset selection problem, giving rise to so-called "Anti-Backdoor Coreset Selection." Since poisonous samples have (a) lower prediction uncertainty and are (b) less frequent than benign samples, coreset selection naturally focuses more on samples associated with benign functionality than the backdoor functionality. We use the Cumulative Entropy as selection criterion to further facilitate this effect. The metric tracks the learning dynamics of training samples and allowing us to select benign samples with high informativeness for the coreset. Additionally, we unlearn the chosen samples in each epoch to facilitate the separability between benign and poisonous samples. Together, this yields an exceptionally effective training-time defense that constructs a benign coreset to train a backdoor-free model. Unlike prior defenses that compromise natural accuracy and fail against certain attacks, our method mitigates backdooring attacks consistently with a negligible impact on natural performance.

==> add_notes.tex <==
\begin{revisionblock}
QUESTIONS:

\begin{itemize}
	\item Why the subset selection by ADAM can be transfered to the final training that uses SGD?
	
	\item If many noised samples are extracted into the final subset, they acts to suppress the backdoor for sure. But does this mean a good defense? Or it is actually not a good purification?
\end{itemize}
\end{revisionblock}

\begin{revisionblock}
UPDATE:

\begin{itemize}
	\item Warm-Up
	using label-smoothing with factor \num{0.1}
	
	(In fact, without using smoothing, the over-fitting will make the training on the final subset quit unstable)
	
	\item Unlearning
	\begin{itemize}
		\item Unlearning set: uniform cross all classes with class-wise size equal the lowest class in the prefix subset pool
		
		\item Unlearning method: retrain with label-smoothing
		
		(Avoid any bias caused by the imbalance of class-wise distribution, \ie the amount discrepancy across classes)
		
		In addition, smoothed retraining on samples with high uncertainty makes the relatively easy classes less unlearned, which is opposite to the hard classes. Concretely, the small number of samples in the intermediate subset indicates an easier learning on the corresponding class. By evenly sampling the same amount sample from each class alone the descending uncertainty order, the mean uncertainty of hard classes will be higher than others.	
		Thus, with the even data amount distribution, the unlearning impact on each class aligns with their learning difficulty, making a further boost of class-wise imbalance in the subset sampling.
		
		\item Unlearning stabilization: $l_2$ regularization between the model before (\ie $\params$) and after unlearning (\ie $\params_{ul}$). The additional regularization loss is defined as: 
		$\loss_{reg} = \sum_{j} \left(\params_{ul}^{(j)} - \params^{(j)}\right)^2$
		
		Why using $l2$ regularization rather $l_2$-norm? 
		
		\textbf{Gradient Simplicity}
		
		Consider a weight vector difference \( x = w - w_0 \), where \( w_0 \) is the reference model (e.g., the model without the data to be forgotten).
		
		\begin{itemize}
			\item The gradient of the squared L2 norm is:
			\[
			\nabla_x \|x\|_2^2 = \nabla_x (x^\top x) = 2x
			\]
			This is simple, smooth, and well-behaved even when \( x \) is close to zero.
			
			\item The gradient of the plain L2 norm is:
			\[
			\nabla_x \|x\|_2 = \nabla_x \sqrt{x^\top x} = \frac{x}{\|x\|_2}
			\]
			This becomes unstable as \( \|x\|_2 \to 0 \), due to division by very small values.
			
		\end{itemize}
		
		Therefore, using the squared L2 norm in regularization leads to more stable and efficient optimization.
		
		\textbf{Quadratic Growth for Penalization}
		
		When applying regularization during training, we want large deviations from the reference model to be penalized more strongly.
		
		\begin{itemize}
			\item The plain L2 norm grows linearly:
			\[
			\|x\|_2 \propto |x|
			\]
			This results in a gentler penalty for larger deviations, which may not be sufficient to enforce strong similarity to the reference model.
			
			\item The squared L2 norm grows quadratically:
			\[
			\|x\|_2^2 \propto x^2
			\]
			This leads to a stronger penalization of larger deviations, effectively pulling the model parameters closer to the reference model.
			
		\end{itemize}
		
		Quadratic growth ensures that the cost of diverging far from the target increases rapidly, making it more effective for regularization in machine unlearning.
		
	\end{itemize}
\end{itemize}
\end{revisionblock}

\begin{revisionblock}
	Target problems:
	
	\begin{itemize}
		\item Informativity of the sampled coreset
		
		\item Stablization of the backdoor learning
		
		\item Representative for the original dataset 
		
		(class-wise distribution)
	\end{itemize}
\end{revisionblock}

\begin{revisionblock}
	Motivation:
	
	\begin{itemize}
		\item Learning behavior of backdoors has to be stable and solid cross all training epochs.
		
		\ie backdoors are easy-to-learn to the certain extend.
	\end{itemize}
\end{revisionblock}

\begin{revisionblock}
	Discussion:
	
	\begin{itemize}
		\item Present isolation performance by uncertainty-based, loss-based, and gradient-based
		
		\item Does the class-wise distribution matter?
		
		(Quantitative or sample-wise?)
		
		\item Why AL is a strong baseline for subset selection?
		
		Defeat the sampling occasionality via multi-cycle subset selection
		
		\item Balance or imbalance?
		
		Balance -> beneficial for a small subset
		
		Imbalance -> beneficial for a large subset
		
		\iffalse
		\item Easy-to-learn vs. hard-to-learn
		
		Easy: important for small set (class centroids)
		
		Hard: important for large set (decision boundary)
		
		\textbullet~ From Top-25k hard:
		\begin{itemize}
			\item Easy subset (1k): 49.52\%
			
			\item Easy subset (2k): 65.29\%
			
			\item Easy subset (2.5k): 71.44\%
			
			\item Easy subset (3k): 73.09\%
			
			\item Easy subset (4k): 77.01\%
			
			\item Easy subset (5k): 82.99\%
			
			\item Easy subset (10k): 89.27\%
			
			\item Easy subset (15k): 91.28\%
			
		\end{itemize}
		
		\textbullet~ From Top-20k hard:
		
		\begin{itemize}
			\item Easy subset (1k): 44.13\%
			
			\item Easy subset (2k): 52.07\%
			
			\item Easy subset (2.5k): 58.83\%
			
			\item Easy subset (3k): 63.94\%
			
			\item Easy subset (5k): 83.69\%
			
			\item Easy subset (10k): 89.94\%
			
			\item Easy subset (15k): 92.65\%
		\end{itemize}
		\fi
		
		\item Select subset for post-train fine-tuning?
		
		\item If sampling a coreset as the given training set, does the poisoning harm the natural performance a lot?
	\end{itemize}
\end{revisionblock}

\begin{revisionblock}
	Evaluation:
	
	\begin{itemize}
		\item Comparing AL with Accumulative Entropy
		
		IoU and Class-wise distribution
		
		\item Comparing the class-wise accuracy to the one by training on entire dataset (mean value \& std value)
		
		\item t-SNE for the entire dataset and the subset
		
		\item Adaptive attack:
		
		Naive training satisfies $\asr \approx \perc{100}$
		
		Using \ourmethod: $\asr \uparrow$
	\end{itemize}
\end{revisionblock}

==> tables/adaptattack_table.tex <==
\newcommand{\adaptcsvreader}[2]{%
	\csvreader[
	head to column names,
	filter = 
	\equal{\Dataset}{#1} 
	\and \not \equal{\Attack}{#2}
	,
	late after line=\\,
	]%
	{res/adapt_attack.csv}%
	{}%
	{%	
		\attacktxt
		& \allnoacc
		& \allnoaccstd
		& \allacc
		& \allaccstd
		%
		& \allnoasr
		& \allnoasrstd
		& \allasr
		& \allasrstd
		%
		& \corenoacc
		& \corenoaccstd
		& \coreacc
		& \coreaccstd
		%
		& \corenoasr
		& \corenoasrstd
		& \coreasr
		& \coreasrstd
	}
}

\begin{adaptivetable}{.9\linewidth}
	\adaptcsvreader{cifar10}{clb}
	\bottomrule
\end{adaptivetable}
